Fair Exploration via Axiomatic Bargaining

Exploration is often necessary in online learning to maximize long-term reward, but it comes at the cost of short-term 'regret'. We study how this cost of exploration is shared across multiple groups. For example, in a clinical trial setting, patients who are assigned a sub-optimal treatment effectively incur the cost of exploration. When patients are associated with natural groups on the basis of, say, race or age, it is natural to ask whether the cost of exploration borne by any single group is 'fair'. So motivated, we introduce the 'grouped' bandit model. We leverage the theory of axiomatic bargaining, and the Nash bargaining solution in particular, to formalize what might constitute a fair division of the cost of exploration across groups. On the one hand, we show that any regret-optimal policy strikingly results in the least fair outcome: such policies will perversely leverage the most 'disadvantaged' groups when they can. More constructively, we derive policies that are optimally fair and simultaneously enjoy a small 'price of fairness'. We illustrate the relative merits of our algorithmic framework with a case study on contextual bandits for warfarin dosing where we are concerned with the cost of exploration across multiple races and age groups.

==> sections/contextual_linear_bandit_long_version.tex <==

\subsection{Regret-Optimal Algorithm for Linear Contextual Bandits (OAM)}
\cite{hao2020adaptive} shows that any consistent algorithm must satisfy the following constraint:
\begin{align} \label{eq:contextual_linear_constraint}
\limsupT \log T ||a||_{\bar{G}_T^{-1}}^2 \leq \frac{\Delta(m, a)^2}{2} \quad \forall m \in [M], a \in \cA(m),
\end{align}
where $\bar{G}_T = \bE\left[\sumt A_t A_t^\top\right]$.
By letting $Q(a) \log T$ represent the total number of times that arm $a$ is pulled, 
we define the following polytope that captures the constraint \eqref{eq:contextual_linear_constraint}:
\begin{align*}
\cQ = \bigg\{ (Q(a))_{a \in \cA} \geq 0 : 
||a||_{H_Q^{-1}}^2 \leq \frac{\Delta(m, a)^2}{2} \; \forall m \in [M], a \in \cA(m), 
H_Q = \sum_{a \in \cA} Q(a) a a^{\top} \bigg\}.
% Q(a) &\geq 0 \; \forall a \in \cA \bigg\}.
\end{align*}
This polytope can be thought of as a re-parameterization of the space of policies, akin to the re-parameterization described in \cref{sec:reparameterize} for $\PFUCB$.
Each element in $\cQ$ represents a possible consistent policy that satisfies $\limT \frac{N_T(a)}{\log T} = Q(a)$ for every $a$.
Then, an instance-dependent lower bound can be constructed by minimizing regret over the space $\cQ$.
Specifically, for any instance $\cI$ and consistent policy $\pi$,
\begin{align} \label{eq:contextual_lower_bound}
\liminfT \frac{\ER_T(\pi, \cI)}{ \log T} \geq Y(\cM, \Delta),
\end{align}
where $Y(\cM, \Delta)$ is the optimal value of the following optimization problem:
\begin{equation}
\begin{aligned} 
Y(\cM, \Delta) = \min_{Q \geq 0} & \sum_{m \in \cM} \sum_{a \in \cA(m)} Q(m, a) \Delta(m, a)\\
\text{s.t. } 
\quad
& Q(a) = \sum_{m : a \in \cA(m)} Q(m, a) \quad \forall a \in \cA \\
& (Q(a))_{a \in \cA} \in \cQ.
% & Q(m, a) \geq 0  \quad \forall  m \in \cM, a \in \cA.
\end{aligned} 
\tag{$L$} \label{eq:contextual_opt_min_regret}
\end{equation}
A feasible solution to \eqref{eq:contextual_opt_min_regret} represents a policy in which the number of times context $m$ pulls arm $a$ is $Q(m, a) \log T$. 
Since context $m$ pulling arm $a$ incurs a regret of $\Delta(m, a)$, the objective function represents log-scaled regret.
$Q(a)$ represents the total number of times that arm $a$ is pulled across contexts, and a consistent policy must satisfy $Q(a) \in \cQ$.

% \subsubsection{Empirical Version of \eqref{eq:contextual_opt_min_regret}}
\textbf{Empirical Version of \eqref{eq:contextual_opt_min_regret}:}
Note that solving the optimization problem \eqref{eq:contextual_opt_min_regret} requires knowledge of $\Delta(m, a)$, which is a function of the true parameter $\theta$.
We describe an empirical version of \eqref{eq:contextual_opt_min_regret} that is solved as part of the OAM algorithm.
At time $t$, let $G_t = \sum_{s=1}^t A_s A_s^{\top}$ and let $\htheta_t = G_t^{-1} \sum_{s=1}^t A_s Y_s$ be the least squares estimate of $\theta$ at time $t$.
Let $\hDelta_t(m, a) = \max_{a' \in \cA(m)} \langle a' - a, \htheta_t \rangle$ be the corresponding estimate of $\Delta(m, a)$.
Let $(\hat{L}_t)$ be the optimization identical to \eqref{eq:contextual_opt_min_regret}, but where $\Delta(m, a)$ is replaced by $\hDelta_t(m, a)$.

% \subsubsection{OAM Outline}
\textbf{OAM Outline:}
We now provide an outline of OAM that captures the main idea of the algorithm; a complete description can be found in \cref{app:oam_alg} or in \cite{hao2020adaptive}.
At each time step $t$, OAM performs the following steps:
\begin{enumerate}
	\item Compute the solution $\hQ_t(m, a)$ of the empirical optimization problem $(\hat{L}_t)$.
	% \item Check if there is an available arm whose number of pulls do not meet this solution, i.e. check if there exists  $N^m_t(a) < $
	\item If there is an available arm $a \in \cA(m_t)$ whose current number of pulls from context $m_t$ is fewer than given by the solution (i.e. $N_t(m_t, a) < \hQ_t(m_t, a) \log T$), then pull this arm.
	\item Otherwise, pull the greedy arm, $\argmax_{a \in \cA(m_t)} \langle a, \htheta_t \rangle$.
\end{enumerate}
There are many details omitted in the above description of the algorithm; refer to \cref{app:oam_alg} for the full description.
The main result from \cite{hao2020adaptive} is that the asymptotic regret of this policy matches the the lower bound \eqref{eq:contextual_lower_bound}.

\subsection{Proportionally Fair OAM (PF-OAM)}

We modify OAM to be a proportionally fair algorithm, by modifying the optimization problem \eqref{eq:contextual_opt_min_regret} that is solved at each time step.
Specifically, we replace the objective function of \eqref{eq:contextual_opt_min_regret} to maximize proportional fairness, rather than minimize regret.

To write down this objective, we first need the single-group regret for each group $g$.
If each group $g$ were by itself, this is equivalent to a linear contextual bandit problem with context distribution $P^g$.
Let $\cM^g \subseteq [M]$ be support of the distribution $P^g$.
Then, $Y(\cM^g, \Delta)$ represents the single-group regret for group $g$.
We can use this to formulate the optimization problem to maximize proportional fairness: 
\begin{equation}
\begin{aligned} 
% Y^{\textrm{fair}} = 
\max_{s, Q \geq 0} & \prod_{g \in \cG} s^g  \\
\text{s.t. } 
\quad
& s^g = \left(Y(\cM^g, \Delta) - \sum_{m \in \cM^g} \sum_{a \in \cA(m)} Q^g(m, a) \Delta(m, a) \right) \\
& Q(a) = \sum_{g \in \cG} \sum_{m : a \in \cA(m)} Q^g(m, a) \quad \forall a \in \cA \\
& (Q(a))_{a \in \cA} \in \cQ \\
& Q^g(m, a) = 0  \quad \forall  g \in \cG, m \notin \cM^g, a \in \cA.
% & Q^g(m, a) \geq 0  \quad \forall  g \in \cG, m \in \cM, a \in \cA \\
% & s^g \geq 0 \quad \forall g \in \cG.
\end{aligned} 
\tag{$L^{\mathrm{fair}}$} \label{eq:contextual_opt_fair}
\end{equation}

\eqref{eq:contextual_opt_fair} has two main differences with \eqref{eq:contextual_opt_min_regret}.
The first is that we now have variables $Q^g(m, a)$ which correspond to how often context $m$ from group $g$ should pull arm $a$.
$Q(a)$ still represents the total number of times that arm $a$ must be pulled, and requiring $Q(a) \in \cQ$ ensures the policy is consistent.
The second difference is that the objective is to maximize proportional fairness, rather than minimize regret.
Solving \eqref{eq:contextual_opt_fair} requires first solving \eqref{eq:contextual_opt_min_regret} for each group $g \in \cG$ to obtain $Y(\cM^g, \Delta)$.
Let $(\hL_t^{\mathrm{fair}})$ be the empirical version of \eqref{eq:contextual_opt_fair}, where $\Delta$ is replaced with $\hDelta_t$.
Then, PF-OAM runs the same steps as OAM with the following two modifications:
\begin{enumerate}
	\item PF-UCB solves $(\hL_t^{\mathrm{fair}})$ rather than $(\hL_t)$.
	\item The condition to check whether to pull an arm $a$ is $N^{g_t}_t(m_t, a) < \hQ_t^{g_t}(m_t, a)$.
\end{enumerate}
All other aspects of the policy remain the same as OAM.

By construction of the optimization problem, it is easy to see that the objective value of \eqref{eq:contextual_opt_fair} is at least as large as the Nash social welfare of all consistent policies.
Proving that PF-OAM exactly achieves this welfare is deferred to future work. 



% This was the first version.
\iffalse
\noindent \textbf{Regret Optimal Policy:}
\cite{hao2020adaptive} provides an instance-dependent lower bound for the linear contextual bandit problem as the optimal value of the following optimization problem:
\begin{equation}
\begin{aligned} 
Y(\cM, \Delta) = \min_{Q \geq 0} & \sum_{m \in \cM} \sum_{a \in \cA(m)} Q(m, a) \Delta(m, a)\\
\text{s.t. } 
\quad
& Q(a) = \sum_{m : a \in \cA(m)} Q(m, a) \quad \forall a \in \cA \\
& (Q(a))_{a \in \cA} \in \cQ.
% & Q(m, a) \geq 0  \quad \forall  m \in \cM, a \in \cA.
\end{aligned} 
\tag{$L$} \label{eq:contextual_opt_min_regret}
\end{equation}
where $\cQ$ is the following polytope that ensures consistency of the policy:
\begin{align*}
\cQ = \bigg\{ (Q(a))_{a \in \cA} \geq 0 : 
||a||_{H_Q^{-1}}^2 \leq \frac{\Delta(m, a)^2}{2} \; \forall m \in [M], a \in \cA(m), 
H_Q = \sum_{a \in \cA} Q(a) a a^{\top} \bigg\}.
% Q(a) &\geq 0 \; \forall a \in \cA \bigg\}.
\end{align*}
\cite{hao2020adaptive} provides a policy (OAM) whose regret matches this lower bound.

The Optimal Allocation Matching (OAM) policy \cite{hao2020adaptive} is regret optimal for the linear contextual bandit model.
OAM works similarly to $\PFUCB$ in that at each time step, 
it solves the empirical optimization problem TODO and then `follows' the solution.
There are many details in OAM that make the policy more complex than $\PFUCB$, including a forced exploration step. The full description of OAM can be found in \cref{app:grouped_linear_contextual_bandit}.

\noindent \textbf{Candidate Fair Policy:}
We propose a fair policy, PF-OAM, which simply runs OAM with a different optimization problem.
Specifically, the objective is replaced from minimizing regret to maximizing Nash SW.
The details can be found in \cref{app:oam_alg}.
\begin{equation}
\begin{aligned} 
% Y^{\textrm{fair}} = 
\max_{s, Q \geq 0} & \prod_{g \in \cG} s^g  \\
\text{s.t. } 
\quad
& s^g = \left(Y(\cM^g, \Delta) - \sum_{m \in \cM^g} \sum_{a \in \cA(m)} Q^g(m, a) \Delta(m, a) \right) \\
& Q(a) = \sum_{g \in \cG} \sum_{m : a \in \cA(m)} Q^g(m, a) \quad \forall a \in \cA \\
& (Q(a))_{a \in \cA} \in \cQ \\
& Q^g(m, a) = 0  \quad \forall  g \in \cG, m \notin \cM^g, a \in \cA.
% & Q^g(m, a) \geq 0  \quad \forall  g \in \cG, m \in \cM, a \in \cA \\
% & s^g \geq 0 \quad \forall g \in \cG.
\end{aligned} 
\tag{$L^{\mathrm{fair}}$} \label{eq:contextual_opt_fair}
\end{equation}
\fi



==> sections/extended_abstract.tex <==
%!TEX root=../paper_fair_bandit.tex

The act of exploring, rather than exploiting, is often necessary to maximize long-term reward in an online learning problem, but it comes at the cost of reducing immediate reward. In a system where the rewards affect different stakeholders, this cost of exploration must be distributed between them in some way. We study a bandit setting where each time step corresponds to a \ii{group}, and the reward of the action represents the utility gained by that group.
% For example, in a healthcare setting, groups can correspond to the race of patients, actions can represent different treatments, and the reward would be the efficacy of the treatment for that patient.
For example, in a setting where a central controller matches users to services (e.g. matching patients to medical specialists), groups can correspond to different types of users (e.g. race), actions can represent the different services, and rewards can correspond to the satisfaction level of the users. This paper studies how to fairly apportion the burden of exploration among the groups of users.

% We study a bandit setting where each time step corresponds a group, a centralized decision maker assigns an action, and the resulting reward represents the utility gained by that group. For example, in a healthcare setting, groups can correspond to different types of patients, the actions can represent different treatments, and the reward would be the efficacy of the treatment for that patient. In this grouped bandit setting, we establish a framework to determine how to fairly share the burden of exploration among the groups.

We use the notion of \ii{proportional fairness} from the well-studied cooperative bargaining framework of \cite{nash1950bargaining}.
We introduce and analyze the grouped $K$-armed bandit model, a simple extension of the classical $K$-armed bandit model where there is an additional bipartite graph that specify which actions a group has access to.
In terms of total regret, we prove that a canonical UCB policy is optimal.
% In terms of \ii{total} regret, we prove that a canonical UCB policy is optimal, in that its regret matches the problem-dependent lower bound.
However, we show that any regret-optimal policy results in an arbitrarily unfair outcome; specifically, such a policy ends up assigning the entire cost of exploration to the group with the most constrained set of options.
We introduce a policy, $\PFUCB$, which we prove to be proportionally fair for all instances, and we show that the loss in total utility as compared to the system optimal solution is a constant for a special class of instances.
Using a real-world dataset on optimal drug dosing where groups correspond to the race of patients, we find that incorporating fairness has a significant impact on the resulting distribution of regret between groups.


% We show that a canonical UCB policy is optimal in terms of \ii{total regret}, but results in an arbitrarily unfair outcome.
% Specifically, we show that any regret-optimal policy ends up assigning the entire cost of exploration to the group that is the most constrained.

% We show that any regret-optimal policy results in an arbitrarily unfair outcome, and therefore total regret must increase in order to obtain a fairer result.
% We introduce a policy, $\PFUCB$, which we prove to be proportionally fair for all instances, and we show that the total regret incurred is only a constant factor higher than the optimal total regret for a special class of instances.



==> sections/intro_old.tex <==

\textbf{Talk about fairness in ML, talk about bandits, and how exploration is a cost: } 

\textbf{Introduce model in words: }
We introduce and study the \ii{grouped bandit} model, a simple extension of the classical $K$-armed bandit model. % There are a set of $G$ groups, and different groups have access to different subsets of arms.
There are $K$ arms and $G$ groups, and there is an known, arbitrary bipartite graph between groups and arms that determine which arms a group has access to.
% One group arrives at each time step, and it must pull one of the arm that it is connected to.
One group arrives at each time step, and a central decision maker must pull one of the arms that the group is connected to.
Regret is measured with respect to the best arm available for that group, and we say that the regret is incurred by the group that arrived.
% We introduce the notion of \ii{group regret}, which refers to the profile of regret incurred by each group.

\textbf{Give 3-armed bandit example: }
The idea of our model and the problems that arise from it can be seen through the following simple example involving three arms and two groups.
\begin{example}[3-armed bandit] \label{ex:3arm}
Suppose there are two groups A and B, and there are three arms with mean rewards $\theta, \theta^A$, and $\theta^B$. 
We will refer to arms by their mean reward.
Group A has access to arms $\theta$ and $\theta^A$, while group B has access to arms $\theta$ and $\theta^B$.
One of the two groups arrive at each time step, where each group arrives with probability 50\%.
Suppose the true parameters satisfy $\theta < \theta^A < \theta^B$, and for simplicity, assume that the mean rewards $\theta^A$ and $\theta^B$ are \ii{known} a priori.
\end{example}

In this setting, the only unknown parameter is $\theta$, and this arm is shared between the two groups.
A reasonable bandit algorithm must pull $\theta$ enough times (i.e. explore enough) to distinguish that it is worse than the other two arms.
When group A pulls $\theta$, the regret incurred is $\theta^A - \theta$, whereas if group B pulls $\theta$, the regret incurred is larger: $\theta^B - \theta$.
Then, it is intuitive that to minimize total regret, 
% it is better for the exploration to happen with group A rather than with group B.
it is better for group A to do the exploration and pull $\theta$ rather than for group B to do so.
% We show that this intuition is correct --- total regret is minimized when group A does all of the exploration, and we show that a canonical UCB algorithm achieves this.
% However, such an algorithm may not be desirable when evaluating \ii{group regret}.
% However, such an algorithm will result in a wildly uneven profile of group regret; group A will incur all of the exploration cost, while group B 
% With this in mind, one may try to devise an algorithm such that we only pull $\theta$ with group A.
Our first result is that we show that a canonical UCB algorithm carries out this intuition.
That is, in this example, we show that a UCB algorithm (namely, KL-UCB of \cite{garivier2011kl}) will result in almost all of the pulls of $\theta$ coming from group A than group B.
We show that this algorithm is optimal, in that we show a problem-dependent lower bound that matches the upper bound on total regret to the exact constant.

However, this ``optimal'' algorithm results in group A incurring essentially all of the total regret, and group B incurring none.
We show that this phenomenon occurs in the general grouped bandit setting --- some groups could incur the majority of the regret while there exist other groups that incur zero regret.
It may be more desirable to distribute the regret in a more ``fair'' manner across the various groups, even if that results in an increase in total regret.

\textbf{Nash Fair Framework: } 
We extend the cooperative bargaining framework, first introduced by Nash (cite), to the bandit setting.
We propose the Nash social welfare function as a fairness metric, also often referred to as \ii{proportional} fairness.
This notion of fairness is often seen as a middle ground between utilitarian (minimize total regret) and min-max fairness (minimize the maximum regret).
% Before describing this fairness metric, we must first introduce the concept of a \ii{disagreement point}.
% In the cooperative bargaining literature, the disagreement point is the value each player can expect to receive if negotiations break down.
% In our group bandit model, we define the disagreement point of a group to be the regret that the group would have incurred if there were no other groups present.
% It can also be described as the regret incurred by each group when no information can be shared between the groups.
% We only consider policies in which the regret of every group is at most its disagreement point, so that all groups benefit by participating.
% Then, the Nash social welfare function is defined as the product of the decrease in regret compared to the disagreement point across the groups. 
We propose an algorithm called $\NFUCB$ which provably maximizes the Nash welfare function asymptotically over all policies.
% This policy ``follows'' the UCB algorithm in terms of determining which arms to pull, but ``splits'' these pulls between groups in a way to maximize the Nash welfare function.

\textbf{Talk about general implications: }

\textbf{List results: } 
We summarize our contributions:
\begin{enumerate}
    \item We introduce the group bandit model and prove a problem-dependent lower bound for the model, analogous to the lower bound of \cite{lai1985asymptotically} for the classical $K$-armed bandit model.
    \item We show that KL-UCB \citep{garivier2011kl} achieves regret that matches the lower bound including constants. 
    % \begin{itemize}
    %     \item Typical UCB analyses involve bounding the \ii{number of pulls} of suboptimal arms. Our result involves analyzing how these pulls are distributed among different groups. For example, in the 3-armed setting, we need to show that essentially all of these pulls of $\theta$ come from group A rather than group B (as well as showing the number of pulls of $\theta$ is optimal, which we essentially get for free from existing UCB analyses).
    % \end{itemize}
    \item We formally define the Nash social welfare function in the grouped bandit model. We introduce the policy \NFUCB, and we show that this policy maximizes the Nash social welfare function over all consistent bandit policies.
\end{enumerate}

\textbf{Talk about proof technique: }
We note that the techniques used in our results are different than the typical techniques used for bandit analyses in the sense that typical analyses involve bounding the \ii{number of pulls} of suboptimal arms, whereas our results involve analyzing \ii{how these pulls are distributed} among different groups. 
For example, to show that KL-UCB is optimal in the 3-armed setting of \cref{ex:3arm}, we need to show that essentially all of these pulls of $\theta$ come from group A rather than group B (as well as showing the number of pulls of $\theta$ is optimal, which we essentially get for free from the existing KL-UCB analysis).




% \textbf{Results in words: }
% We first provide a problem-dependent lower bound for this problem, an extension of the Lai-Robbins lower bound for the canonical $K$-armed bandit model. Then, we show that this lower bound can be matched to the exact constant by running a UCB algorithm. In showing this upper bound, we show exactly how the regret is distributed among the groups. In particular, we show that



\subsection{Literature Review}
\begin{itemize}
    \item $K$-armed bandits, lai robbins
    \item Similar bandits models: Sleeping bandits \cite{kleinberg2010regret}, Manish's paper \cite{raghavan2018externalities}
    \item Fairness: Nash fairness, other fairness papers in ML / operations, other fairness papers in bandits
\end{itemize}

==> sections/proofs_klucb_opt.tex <==
%!TEX root=../paper_fair_bandit.tex

% The existing analysis of KL-UCB proves that the \ii{number of pulls} of a suboptimal arm is optimal:
% \begin{theorem}[Number of suboptimal pulls is optimal.] \label{theorem:number_pulls}
% Let $a \in \cA_{\text{sub}}$ be a suboptimal arm.
% The grouped-KL-UCB algorithm satifies:
% \begin{align}
%  \limsup_{T \rightarrow \infty} \frac{\bE\left[N_T(a)\right] }{\log T}\leq \frac{1}{\KL(\theta_a, \OPT(\gmin(a)))}.
% \end{align}
% \end{theorem}

% To show \cref{thm:klucb_opt_stochastic_arrivals}, we need to analyse how these pulls are distributed across groups.
% We prove that the number of times an arm $a$ gets pulled by a group not in $\gmin(a)$ is $O(\log \log t)$.
% % Let $I_t^g(a)$ be the indicator variable on if group $g$ pulled arm $a$ at time $t$.
% \begin{theorem} \label{thm:main_theorem}
% Let $a \in \cA$. Let $B \in G_a$, $B \notin \gmin(a)$ be a group that has access to the arm but is not the group that has the smallest optimal out of $G_a$.
% Then,
% \begin{align}
% % \lim_{T \rightarrow \infty} \bE\left[\sum_{t=1}^T I_t^B(a)\right] \leq C_3 \log \log T
%  \bE\left[N_T^B(a) \right] = O(\log \log T),
% \end{align}
% where the big-$O$ hides constants that depend on the instance.
% \end{theorem}

% \begin{myproof}[Proof of \cref{thm:klucb_opt_stochastic_arrivals}]
% Recall that $\gmin(a)$ are the set of groups in $G_a$ with the smallest OPT.
% For any $g \in \gmin(a)$, $\OPT(g)$ is the same.
% \begin{align}
% & \limsup_{T \rightarrow \infty}\frac{\bE[\Reg(T, \pi, \cI)]}{\log T} \\
% =& \limsup_{T \rightarrow \infty} \sum_{a \in \cA} \sum_{g \in G_a}  \frac{(\OPT(g) - \theta_a)\bE[N^g_T(a)]}{\log T} \\
% \leq& \limsup_{T \rightarrow \infty} \sum_{a \in \cA} \left( \frac{(\OPT(\gmin(a)) - \theta_a)}{\log T} \sum_{g \in \gmin(a)}  \bE[N^g_T(a)]
%  + \sum_{g \notin \gmin(a)}   \frac{(\OPT(g) - \theta_a)\bE[N^g_T(a)]}{\log T} \right) 
% \end{align}
% From \cref{thm:main_theorem}, if $g \notin \gmin(a)$, $\bE[N^g_T(a)] = O(\log \log T)$, therefore the second term vanishes.
% Also, note that if an arm is not suboptimal, then $\OPT(\gmin(a)) - \theta_a = 0$.
% Using $\sum_{g \in \gmin(a)} \bE[N^g_T(a)] \leq \bE[N_T(a)]$, we get
% \begin{align}
% \limsup_{T \rightarrow \infty}\frac{\bE[\Reg(T, \pi, \cI)]}{\log T} 
% &= \limsup_{T \rightarrow \infty} \sum_{a \in \cA_{\text{sub}}} (\OPT(\gmin(a)) - \theta_a)  \frac{\bE[N_T(a)]}{\log T} \\
% &= \sum_{a \in \cA_{\text{sub}}} \frac{\OPT(\gmin(a)) - \theta_a}{\KL(\theta_a, \OPT(\gmin(a)))},
% \end{align}
% where the last step follows from \cref{theorem:number_pulls}.
% \end{myproof}

\iffalse % TODO: this result abstracts away alot of details
\subsection{Key Results}
\begin{proposition} \label{prop:main_proposition_epochs}
Let $r > 0$ be fixed.
Suppose we run any log-consistent policy.
For any action $a \in \cA$,
\begin{align*}
\sumt \Pr(\pulls(a), \UCB_t(a) \geq \OPT(\gmin(a)) + r) = O(\log \log T),
\end{align*}
where the constant in the big-$O$ may depend on the instance and $r$.
\end{proposition}

\begin{myproof}[Proof of \cref{prop:main_proposition_epochs}]
TODO
\end{myproof}
\fi


% This proof can be broken down into two steps.
The first step of the proof is to show that the \ii{number of pulls} of a suboptimal arm is optimal:
\begin{theorem} \label{theorem:number_pulls}
Let $a \in \cA_{\text{sub}}$ be a suboptimal arm.
KL-UCB satisfies
\begin{align*}
 \limsup_{T \rightarrow \infty} \frac{\bE\left[N_T(a)\right] }{\log T}
 % \leq \frac{1}{\KL(\theta_a, \OPT(\gmin(a)))}.
 \leq \Nopta.
\end{align*}
\end{theorem}
This result can be shown using the existing analysis of KL-UCB from \cite{garivier2011kl}.
% To show \cref{thm:klucb_opt_stochastic_arrivals}, 
The next step is to analyze how these pulls are distributed across groups.
% In particular, we need to show that for any suboptimal arm $a$, all of its pulls come from a group in $\gmin(a)$.
In particular, we need to show that a group never pulls a suboptimal arm $a$ if $g \notin \gmin(a)$.
% In particular, we need to show that regret is incurred by a group $g$ pulling arm $a$ only when $g \in \gmin(a)$.
This is the result of the next theorem:
% We prove that the number of times an arm $a$ gets pulled by a group not in $\gmin(a)$ is $O(\log \log t)$:
% Let $I_t^g(a)$ be the indicator variable on if group $g$ pulled arm $a$ at time $t$.
\begin{theorem} \label{thm:main_theorem}
Let $a \in \cA$. Let $g \in G_a$, $g \notin \gmin(a)$ be a group that has access to the arm but is not the group that has the smallest optimal out of $G_a$.
Then, KL-UCB satisfies
\begin{align*}
% \lim_{T \rightarrow \infty} \bE\left[\sum_{t=1}^T I_t^B(a)\right] \leq C_3 \log \log T
 \bE\left[N_T^g(a) \right] = O(\log \log T),
\end{align*}
where the big-$O$ hides constants that depend on the instance.
\end{theorem}

This result implies that for any arm $a$, the regret incurred by group $g \notin \gmin(a)$ pulling the arm is $o(\log T)$, and is equal to 0 when scaled by $\log T$.
\cref{thm:klucb_opt_stochastic_arrivals} then follows from combining \cref{theorem:number_pulls} and \cref{thm:main_theorem}.

In this section, we prove \cref{thm:main_theorem}.
% We prove this result for an arm $a \in \cA_{\text{sub}}$; i.e. $a$ is not optimal for any group.
% The result for an arm $a \notin \cA_{\text{sub}}$ follows the same steps with a couple small tweaks and is described in \cref{sec:proof_optimal_arm}.
% Fix an instance $\cI =(\theta, \cG, \cA, (p_g)_{g \in \cG}, (\cA_g)_{g \in \cG})$.
Let $a \in \cA$ and let $A \in \gmin(a)$ be a group that has access to that arm with the smallest OPT.
Let group $B \notin \gmin(a)$ be another group that has access to arm $a$.
Let $\thetaA, \thetaB$ be the optimal arms for group A and B respectively. 
We use $\thetaA, \thetaB$ to refer to both the arm and the arm means.
Our goal is to show $\bE\left[N_T^B(a) \right] = O(\log \log T)$.

% Let $\pulls^g(a)$ be the indicator for when group $g$ has pulled arm $a$ at time $t$ (it must be that group $g$ arrived for this event to happen). Then,
\begin{align*}
\bE\left[N_T^B(a) \right]
&= \sum_{t=1}^T \Pr(\pulls^B(a)) \\
 % = \sum_{t=1}^T \Pr(I^B_\theta(t), J_t) + \sum_{t=1}^T \Pr(I^B_\theta(t), \bar{J}_t)
& = \sum_{t=1}^T \Pr(\pulls^B(a),  \UCB_t(\thetaB) \geq \thetaB)
     % &\quad + \sum_{t=1}^T \Pr(\pulls^B(a), \hthetat > \theta_u)
      + \sum_{t=1}^T \Pr(\pulls^B(a), \UCB_t(\thetaB) < \thetaB).
\end{align*}

The second sum can be bounded by \cref{commonlemma:allucb}, since 
$ \sumt \Pr(\pulls^B(a), \UCB_t(\thetaB) < \thetaB) \leq \sumt \Pr(\notallucb_t) = O(\log \log T)$.
% From \cref{commonlemma:empirical_mean_close_when_pulled}, $\sumt \Pr(\pulls^B(a), \hthetat > \theta_u)  = O(1)$.
Therefore, our goal is to show 
\begin{align} \label{eq:klopt_main_eq}
\sumt \Pr(\pulls^B(a),  \UCB_t(\thetaB) \geq \thetaB) = O(\log \log T).
\end{align}

We state a slightly more general result that implies \eqref{eq:klopt_main_eq}.
\begin{lemma} \label{lemma:main_epoch}
Suppose we run any log-consistent policy $\pi$.
Let $r > 0$ be fixed.
For any $a \in \cA$,
\begin{align*}
\sumt \Pr(\pulls(a), \UCB_t(a) \geq \OPT(\gmin(a)) + r) = O(\log \log T),
\end{align*}
where the constant in the big-$O$ may depend on the instance and $r$.
\end{lemma}
The rest of this section proves \cref{lemma:main_epoch}.


\iffalse
We bound each of the three sums separately, which proves our main result.
\begin{lemma} \label{lemma:klucb_E_t}
   $\sum_{t=1}^T \Pr(E_t) = O(\log \log T)$.
\end{lemma}
\begin{lemma} \label{lemma:klucb_UCB}
   $\sum_{t=1}^T \Pr(\pulls^B(a), \UCB_t(B) < \thetaB) = O (\log \log T)$.
\end{lemma}
\begin{lemma} \label{lemma:klucb_empirical_mean}
   $\sum_{t=1}^T \Pr(\pulls^B(a), \hthetat > \theta_u) = O(1)$.
\end{lemma}

The crux of the analysis is in \cref{lemma:klucb_E_t}, which we prove in \cref{sec:main_lemma_proof}.
\cref{lemma:klucb_UCB} follows from Theorem 10 of \cite{garivier2011kl}, and
\cref{lemma:klucb_empirical_mean} follows from the fact that the tail of $\hthetat$ decays exponentially in the number of pulls of $a$ (Proof is in \cref{sec:pf_mean_lemma}).
\fi


\subsection{Probabilistic Lower Bound of $N_t(a)$ for Grouped Bandit}

One of the main tools used in the proof of \cref{lemma:main_epoch} is a high probability lower bound on the number of pulls of a suboptimal arm.
% Given a group $g$, our result is a probabilistic lower bound on the number of pulls of a suboptimal arm $j$.
Let $\arr$ be the number of arrivals of group $g$ by time $t$.
Let $R^g_t = \{\arr \geq \frac{p_g t}{2}\}$ be the event that the number of arrivals of group $g$ is at least half of the expected value.
We condition on the event $R^g_t$ to ensure that a group has arrived a sufficient number of times.
\begin{proposition}  \label{prop:lower_bound_stochastic}
Let $g$ be a group, and let $a \in \Asubg$ be a suboptimal arm for group $g$.
Fix $\eps \in (0, 1)$.
Suppose we run a log-consistent policy as defined in \cref{def:log_consistent}.
Then,
\begin{align*}
\Pr\left(N_{t}(a) \leq \frac{(1-\eps)\log t}{\KL(\theta(a), \OPT(g))}  \;\bigg|\; R^g_t  \right) = O\left(\frac{1}{\log t}\right),
\end{align*}
where the big-$O$ notation is with respect to $t \rightarrow \infty$.
\end{proposition}
The proof of this result can be found in \cref{sec:proof_lower_bound_stochastic}.
For an arm $a \notin \cA_{\text{sub}}$, we have the following stronger result:
\begin{proposition}  \label{prop:lower_bound_opt_stochastic}
Let $a$ be an arm that is optimal for some group $g$.
Suppose we run a log-consistent policy.
Then, for any $b > 0$,
\begin{align*}
\Pr\left(N_t(a) \leq b \log t \;\big|\; R^g_t\right) = O\left(\frac{1}{\log t}\right),
\end{align*}
where the big-$O$ notation is with respect to $t \rightarrow \infty$ and hide constants that depend on both $b$ and the instance.
\end{proposition}



\subsection{Proof of \cref{lemma:main_epoch}} \label{sec:main_lemma_proof}
\textbf{Outline:} 
Let $A \in \gmin(a)$ be a group that has the smallest optimal out of all arms with access to $a$.
The main idea of this lemma is that group A does not ``allow'' the UCB of arm $a$ to grow as large as $\OPT(A) + r$, as group A would pull arm $a$ once the UCB is above $\OPT(A)$.
\cref{prop:lower_bound_stochastic} implies that $\UCB_t(a)$ is not larger than $\OPT(A)$ with high probability.
If this occurs at time $t$, since the radius of the UCB grows slowly (logarithmically), the earliest time that the UCB can grow to $\OPT(A) +r$ is $t^\gamma$, for some $\gamma > 1$.
We divide the time steps into epochs, where if epoch $k$ starts at time $s_k$, it ends at $s_k^\gamma$.
This exponential structure gives us $O(\log \log T)$ epochs in total, and we show that the expected number of times that $\UCB_t(a) > \OPT(A) + r$ during one epoch is $O(1)$.


% First, assume that $a \in \Asub$. 
\noindent \textbf{Proof:}
We denote by $\theta_a$ the true mean reward of arm $a$ and by $\htheta_t$ the empirical mean reward of $a$ at the start of time $t$. 
Let $U = \OPT(\gmin(a)) + r$.
Let $A \in \gmin(a)$, and let $\thetaA = \OPT(A)$.
If $a \notin \Asub$, then let $\thetaA = \OPT(A) + r/2$.
Let $b > 0$ such that $\frac{\KL(\theta_a, U)}{\KL(\theta_a, \thetaA)}= 1+b$.
Define $\theta_u \in [\theta_a, \thetaA]$ such that $\frac{\KL(\theta_u, U)}{\KL(\theta_a, \thetaA)}= 1+\frac{b}{2}$.
We have $\theta_a < \theta_u < \thetaA  < U$.
% Recall that $\frac{\KL(\theta_u, \thetaB)}{\KL(\theta, \thetaA)} = 1+\frac{c}{2}$.
Define $\gamma \triangleq 1+\frac{b}{4}$.
Let $\eps > 0$ such that $\frac{1-\eps}{1+\eps}\cdot \frac{\KL(\theta_u, U)}{\KL(\theta_a, \thetaA)} = \gamma$.

By \cref{commonlemma:empirical_mean_close_when_pulled}, 
$\sumt \Pr(\pulls(a), \htheta_t(a) > \theta_u) = O(1)$.
Therefore, we can assume $\htheta_t(a) \leq \theta_u$.
Denote the event of interest by $E_t = \{\pulls(a), \UCB_t(a) \geq \thetaA + r, \htheta_t(a) \leq \theta_u\}$.
% Denote the event of interest by $E_t = \{\pulls(a), \UCB_t(a) \geq \thetaA + r\}$.
Our goal is to show $\sumt \Pr(E_t) = O(\log \log T)$.



Divide the time interval $T$ into $K = O(\log \log T)$ epochs. %, where epoch $k$ will start at time step $s_k = 2^{\gamma^k}$, where $\gamma > 1$.
Let epoch $k$ start at $s_k \triangleq \left\lceil 2^{\gamma^k}  \right\rceil$ for $k \geq 0$. Let $\cT_k = \{s_k, s_k+1, \dots, s_{k+1}-1\}$ be the time steps in epoch $k$.
This epoch structure satisfies the following properties:
\begin{enumerate}
    \item The total number of epochs is $O(\log \log T)$.
    \item $\frac{\log s_{k+1}}{\log s_k} = \gamma$ for all $k \geq 0$.
\end{enumerate}

We will treat each epoch separately.
Fix an epoch $k$.
Our goal is to bound $ \bE\left[\sum_{t \in \cT_k} \bI(E_t) \right] $.
\cref{commonlemma:ucb_radius_logarithmic_pulls} implies that there exists a constant $c > 0$ such that if $E_t$ occurs, it must be that $N_t(a) < c \log t$.
Hence, 
\begin{align*}
\sum_{t \in \cT_k} \bI(E_t) \leq c \log s_{k+1}.
\end{align*}

Define the event $G_t = \left\{N_{t}(a) \geq (1-\eps)\frac{\log t}{\KL(\mu, \thetaA)}\right\}$.
The following claim says that if $G_{s_k}$ is true, then $E_t$ never happens during that epoch. 
\begin{claim} \label{claim:good_event_epoch}
Suppose $G_{s_k}$ is true.
Let $t_0$ be such that if $t \geq t_0$, $\log \log t \leq \eps \log t$.
Then, if $s_k \geq t_0$,$\sum_{t = s_k}^{s_{k+1}} \bI(E_t) = 0$.
% Then, $E_{t'}$ is false for all time steps $t'$ in epoch $k$.
\end{claim}
This result follows from the fact that the event $G_{s_k}$ implies that the radius of the UCB is ``small'' at time $s_k$, 
and the epoch is defined so that the radius will not grow large enough that $E_t$ can occur during epoch $k$.
Therefore, we have the following:
\begin{align*} 
\bE\left[\sum_{t \in \cT_k} \bI(E_t) \right]
= \bE\left[\sum_{t \in \cT_k} \bI(E_t) \bigg| \bar{G}_{s_k}  \right]
\Pr\left(\bar{G}_{s_k} \right) 
\leq c \log s_{k+1}\Pr\left(\bar{G}_{s_k} \right).
\end{align*}

We can bound $\Pr\left(\bar{G}_{s_k} \right)$ using the probabilistic lower bound of \cref{prop:lower_bound_stochastic}.
\begin{claim} \label{claim:prob_g_h}
$\Pr\left( \bar{G}_{s_k} \right) \leq  O\left(\frac{1}{\log s_{k}}\right)$.
\end{claim}

Then, property 2 of the epoch structure implies 
$\bE\left[\sum_{t \in \cT_k} \bI(E_t) \right] = O(1)$.
Since the number of epochs is $O(\log \log T)$,
% if $k_1 \geq k_0$ is the smallest epoch such that $s_{k_1} \geq t_0$,
\begin{align*}
 \bE\left[\sum_{t = 1}^{T} \bI(E_t)\right]
  \leq \sum_{k=1}^K \bE\left[\sum_{t \in \cT_k} \bI(E_t)\right]
  =O(\log \log T),
\end{align*}
as desired.

% If $a \notin \Asub$, the exact same proof goes through if we replace $\thetaA$ by $\thetaA + r/2$.

\subsection{Proof of Claims} \label{sec:proof_of_claims}

\iffalse
\begin{claim} \label{claim:numpull_must_be_small}
If $E_t$ is true, then
$N_t(\theta) \leq \frac{\log t+ 3 \log \log t}{\KL(\theta_u, \thetaB)}$.
Since $\sum_{s=1}^t \bI(E_s) \leq N_t(\theta)$, and $M_t(B) \leq t$,
$\sum_{s=1}^t \bI(E_s) \leq \frac{\log t + 3 \log \log t}{\KL(\theta_u, \thetaB)}$.
\end{claim}

\begin{myproof}[Proof of \cref{claim:numpull_must_be_small}]
By definition of KL-UCB, we have
\begin{align*}
N_t(a) \leq \frac{\log t + 3 \log \log t}{\KL(\hthetat, \UCB_t(\theta))}.
\end{align*}
For $E_t$ to occur, it must be that $\UCB_t(a) > \thetaB$ and $\hthetat \leq \theta_u$.
The result follows from $\KL(\hthetat, \UCB_t(a)) \geq \KL(\theta_u, \thetaB)$.
% (Uses ``monotone'' property of KL.)
\end{myproof}
\fi


\begin{myproof}[Proof of \cref{claim:good_event_epoch}]
Let $t = s_k > t_0$ and let $t' \geq t$ such that $E_{t'}$ is true.
By definition of KL-UCB,
\begin{align*}
N_{t'}(a) \leq \frac{\log {t'} + 3 \log {t'}}{\KL(\htheta_{t'}, \UCB_{t'}(\theta))}.
\end{align*}
Since $E_{t'}$ implies $\UCB_{t'}(a) > \thetaB$ and $\htheta_{t'} \leq \theta_u$, we have $N_{t'}(a) \leq \frac{\log {t'} + 3 \log {t'}}{\KL(\theta_u, \thetaB)}$.
Since $G_{s_k}$ is true, $N_{t'}(a) \geq (1-\eps)\frac{\log s_k}{\KL(\theta_a, \thetaA)}$.
Therefore, it must be that
\begin{align}
&(1-\eps)\frac{\log s_k}{\KL(\theta_a, \thetaA)}
\leq \frac{\log t' + 3 \log \log t'}{\KL(\theta_u, \thetaB)}
\leq \frac{(1+\eps)\log t'}{\KL(\theta_u, \thetaB)} \nonumber \\
% \Rightarrow\;& \frac{(1-\eps)\KL(\theta_u, \thetaB)\log t}{(1+\eps)\KL(\theta, \thetaA)} \leq  \log t' \\
\Rightarrow\;&\frac{1-\eps}{1+\eps}\cdot \frac{\KL(\theta_u, \thetaB)}{\KL(\theta_a, \thetaA)} \log s_k \leq  \log t' \nonumber \\
\Rightarrow \;& t' \geq s_k^\gamma. \nonumber
\end{align}
This implies that $t'$ is not in epoch $k$.
% Suppose, to the contrary, $t' < s_{k+1}$.
% Since $M_{s_k}(A) > q_A s_k$ and $G_k$ is true, by \cref{eq:good_event_subclaim}:
% \begin{align*}
% M_{t'}(B) 
% &> \left(q_A s_k \right)^{\gamma}
% % &\geq  \left(\frac{q_A}{q_B}\right)^{\gamma + \dots + \gamma^{k+1}} 2^{\gamma^{k+1}}.
% \end{align*}
% Since $t' < s_{k+1}$, $M_{t'}(B) \leq M_{s_{k+1}}(B) \leq q_B (s_{k+1}-1)$.
% This implies 
% \begin{align*}
% s_{k+1} > \frac{1}{q_B} \left(q_a s_k\right)^{\gamma}+1,
% \end{align*}
% which contradicts the definition of $s_{k+1}$.
\end{myproof}

\begin{myproof}[Proof of \cref{claim:prob_g_h}]

For group $g = A$,
\cref{prop:lower_bound_stochastic} (or \cref{prop:lower_bound_opt_stochastic} if $a \notin \Asub$) states that
\begin{align*}
\Pr\left(\bar{G}_{s_k} \vg R_{s_k}^g \right) = O\left(\frac{1}{\log s_k} \right).
\end{align*}
(We show in \cref{app:sec:klucb_log_consistent} that KL-UCB is log-consistent.)

Now we need to bound $\Pr(\bar{R}_{s_k}^g) = \Pr\left( M_{s_k}(A) \leq \frac{p_A s_k}{2}\right)$.
Note that $M_s(A) = \sum_{t=1}^s Z_i^A$, where $Z_t^A \overset{\text{iid}}{\sim} \text{Bern}(p_A)$.
By Hoeffding's inequality,
\begin{align*}
\Pr\left(M_{s_{k}}(A) \leq \frac{p_A s_k}{2}\right) < \exp\left(-\frac{1}{2} p_A^2 s_{k}\right).
\end{align*}

Combining, we have
\begin{align*}
\Pr(\bar{G}_k) 
&\leq \Pr(\bar{R}_k) + \Pr(\bar{G}_k \vv R_k) \leq O\left(\frac{1}{\log s_k}\right).
\end{align*}

\end{myproof}


\iffalse
We first state a result stating that for $E_t$ to happen, it must be that $N_t(\theta)$ must be smaller than a threshold. 
\begin{claim} \label{claim:numpull_must_be_small}
If $E_t$ is true, then
% \begin{align}
$N_t(\theta) \leq \frac{\log t+ 3 \log \log t}{\KL(\theta_u, \thetaB)}$.
% \end{align}
Since $\sum_{s=1}^t \bI(E_s) \leq N_t(\theta)$, and $M_t(B) \leq t$,
$\sum_{s=1}^t \bI(E_s) \leq \frac{\log t + 3 \log \log t}{\KL(\theta_u, \thetaB)}$.
% \begin{align} \label{eq:num_Bt}
% \sum_{s=1}^t \bI(E_s) \leq \frac{\log t + 3 \log \log t}{\KL(\theta_u, \thetaB)}.
% \end{align}
\end{claim}
This result follows from the definition of $E_t$ and the KL-UCB algorithm.
The proof of this and all other claims in this proof can be found in \cref{sec:proof_of_claims}.



% The second result states that if $N_t(\theta)$ is greater than a particular threshold, $E_{t'}$ cannot occur until $t'$ is on the order of $t^{\gamma}$.
% \begin{claim} \label{claim:doubly_exponential}
% Suppose at time $t \geq t_0$, $N_t(\theta) \geq (1-\eps)\frac{\log M_{t}(A)}{\KL(\theta, \thetaA)}$.
% If $E_{t'}$ occurs for some $t' \geq t$, where $M_{t'}(B) \geq t_0$, it must be that $M_{t'}(B) \geq M_t(A)^{\gamma}$.
% \end{claim}
% The proof of this claim simply uses the definition of $G_k$ along with the constraint on $N_t(\theta)$ enforced by \cref{claim:numpull_must_be_small}.

We will divide the time interval $T$ into $K = O(\log \log T)$ epochs. %, where epoch $k$ will start at time step $s_k = 2^{\gamma^k}$, where $\gamma > 1$.
Recall that $\frac{\KL(\theta_u, \thetaB)}{\KL(\theta, \thetaA)} = 1+\frac{c}{2}$.
Define $\gamma \triangleq 1+\frac{c}{4}$.
Let $\eps > 0$ such that $\frac{1-\eps}{1+\eps}\cdot \frac{\KL(\theta_u, \thetaB)}{\KL(\theta_a, \thetaA)} = \gamma$.
% Let $q_A = \frac{p_A}{2}$ and let $q_B = 2 p_B$.
% Let $t_0 \geq 0$ such that if $t \geq t_0$, $3 \log \log t \leq \eps \log t$.
Let epoch $k$ start at $s_k \triangleq \left\lceil 2^{\gamma^k}  \right\rceil$ for $k \geq 0$. Let $\cT_k = \{s_k, s_k+1, \dots, s_{k+1}-1\}$ be the time steps in epoch $k$.
This epoch structure satisfies the following properties:
\begin{enumerate}
    \item The total number of epochs is $O(\log \log T)$.
    \item $\frac{\log s_{k+1}}{\log s_k} = \gamma$ for all $k \geq 0$.
\end{enumerate}
% \begin{claim} \label{claim:epoch_structure}
% \end{claim}

We will treat each epoch separately.
Fix an epoch $k$.
Our goal is to bound $ \bE\left[\sum_{t \in \cT_k} \bI(E_t) \right] $.
Define the event $G_t = \left\{N_{t}(a) \geq (1-\eps)\frac{\log t}{\KL(\theta_a, \thetaA)}\right\}$.
The following claim says that if $G_{s_k}$ is true, then $E_t$ never happens during that epoch.
\begin{claim} \label{claim:good_event_epoch}
Suppose $G_{s_k}$ is true.
Then, $\sum_{t = s_k}^{s_{k+1}} \bI(E_t) = 0$.
% Then, $E_{t'}$ is false for all time steps $t'$ in epoch $k$.
\end{claim}
The proof of this claim simply uses the definition of $G_k$ along with the constraint on $N_{s_k}(\theta)$ enforced by \cref{claim:numpull_must_be_small}.
Therefore, we have the following:
\begin{align} \label{eq:main1}
\bE\left[\sum_{t \in \cT_k} \bI(E_t) \right]
= \bE\left[\sum_{t \in \cT_k} \bI(E_t) \bigg| \bar{G}_{s_k}  \right]
\Pr\left(\bar{G}_{s_k} \right)
\end{align}

\cref{claim:numpull_must_be_small} bounds 
$\sum_{t \in \cT_k} \bI(E_t)$ to be at most $\frac{\log s_{k+1} + 3 \log \log \log s_{k+1}}{\KL(\theta_u, \thetaB)}$.
If $s_{k+1} > t_0$, then $\sum_{t = s_k}^{s_{k+1}} \bI(E_t) \leq \frac{(1+\eps)\log s_{k+1}}{\KL(\theta_u, \thetaB)}$.
 Bounding $\Pr\left(\bar{G}_{s_k} \right)$ comes from the probabilistic lower bound of \cref{prop:lower_bound_stochastic}.
\begin{claim} \label{claim:prob_g_h}
$\Pr\left( \bar{G}_{s_k} \right) \leq  O\left(\frac{1}{\log s_{k}}\right)$.
\end{claim}

Therefore, as long as $s_k \geq t_0$ and $k \geq k_0$, \eqref{eq:main1} can be bounded by
\begin{align*}
 \bE\left[\sum_{t \in \cT_k} \bI(E_t) \right] 
\leq& \frac{(1+\eps)\log s_{k+1}}{\KL(\theta_u, \thetaB)} O\left(\frac{1}{\log s_{k}}\right) \\
% \leq& \frac{(1+\eps)\log s_{k+1}}{\KL(\theta_u, \thetaB)} \left( \Pr\left(\bar{H}_k \right) +  \Pr\left({H}_k, \bar{G}_k \right) \right) \\
 % \leq& \frac{(1 + \eps)\log s_{k+1}}{\KL(\theta_u, \thetaB)} \cdot \frac{C_1}{\log s_{k}} \\
 \leq& \frac{(1 + \eps)}{\KL(\theta_u, \thetaB)}O(1),
\end{align*}
where the last inequality follows from property 2 of the epoch structure.
Since the number of epochs is $O(\log \log T)$,
if $k_1 \geq k_0$ is the smallest epoch such that $s_{k_1} \geq t_0$,
\begin{align*}
 \bE\left[\sum_{t = 1}^{T} \bI(E_t)\right]
  \leq s_{k_1} + \sum_{k=k_1}^K \bE\left[\sum_{t \in \cT_k} \bI(E_t)\right]
  =O(\log \log T),
\end{align*}
as desired.
\fi


